A Progressive Transformer for Unifying Binary Code Embedding and Knowledge Transfer

Language model approaches have recently been integrated into binary analysis tasks, such as function similarity detection and function signature recovery. These models typically employ a two-stage training process: pre-training via Masked Language Modeling (MLM) on machine code and fine-tuning for specific tasks. While MLM helps to understand binary code structures, it ignores essential code characteristics, including control and data flow, which negatively affect model generalization. Recent work leverages domain-specific features (e.g., control flow graphs and dynamic execution traces) in transformer-based approaches to improve binary code semantic understanding. However, this approach involves complex feature engineering, a cumbersome and time-consuming process that can introduce predictive uncertainty when dealing with stripped or obfuscated code, leading to a performance drop. In this paper, we introduce ProTST, a novel transformer-based methodology for binary code embedding. ProTST employs a hierarchical training process based on a unique tree-like structure, where knowledge progressively flows from fundamental tasks at the root to more specialized tasks at the leaves. This progressive teacher-student paradigm allows the model to build upon previously learned knowledge, resulting in high-quality embeddings that can be effectively leveraged for diverse downstream binary analysis tasks. The effectiveness of ProTST is evaluated in seven binary analysis tasks, and the results show that ProTST yields an average validation score (F1, MRR, and Recall@1) improvement of 14.8% compared to traditional two-stage training and an average validation score of 10.7% compared to multimodal two-stage frameworks.

==> files/tables/RQ2_obf.tex <==
\begin{table}[t]
\centering
\caption{Comparison between \system and XDA on different tasks across different obfuscation methods. \berkay{\system and XDA repeats in the table a lot (in each row.). You need to find a better way of presenting these numbers. }}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{l|l|rrr}
\hline
\multirow{2}{*}{Tasks} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Obf. Methods} \\
 &  & bcf & cff & sub \\ \hline
Inst Boun & \system & \multirow{2}{*}{0.862} & \multirow{2}{*}{0.864} & \multirow{2}{*}{0.864} \\
 & XDA &  &  &  \\ \hline
Func Boun & \system & \textbf{0.863} & \textbf{0.813} & \textbf{0.864} \\
 & XDA & 0.394 & 0.546 & 0.529 \\ \hline
Func Sig Count & \system & \textbf{0.654} & \textbf{0.652} & \textbf{0.669} \\
 & XDA & 0.344 & 0.357 & 0.374 \\ \hline
Func Sig Type & \system & \textbf{0.379} & \textbf{0.382} & \textbf{0.439} \\
 & XDA & 0.371 & 0.362 & 0.413 \\ \hline
Func Name & \system & \textbf{0.435} & \textbf{0.447} & \textbf{0.532} \\
 & XDA & 0.391 & 0.383 & 0.482 \\ \hline
Comp Prov & \system & \textbf{0.463} & \textbf{0.488} & \textbf{0.423} \\
 & XDA & 0.412 & 0.421 & 0.387 \\ \hline
Func Sim 32 & \system & \textbf{0.793} & \textbf{0.9} & \textbf{0.908} \\
 & XDA & 0.624 & 0.701 & 0.792 \\ \hline
Func Sim 1000 & \system & \textbf{0.343} & \textbf{0.583} & \textbf{0.601} \\
 & XDA & 0.196 & 0.269 & 0.393 \\ \hline
\end{tabular}%
}
\label{tab: RQ2_robustness_obf}
\end{table}

==> files/tables/RQ2_optimization.tex <==
\begin{table}[t]
\centering
\caption{Comparison between \system and XDA on different tasks across different optimization levels.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrrrrrrr}
\hline
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{8}{c}{\textbf{Optimization}} \\
\multicolumn{1}{l|}{\multirow{-2}{*}{\textbf{Tasks}}} & \multicolumn{1}{l|}{\multirow{-2}{*}{\textbf{Model}}} & \textbf{O0} & \textbf{Od} & \textbf{O1} & \textbf{Ox} & \textbf{O2} & \textbf{Os} & \textbf{O3} & \textbf{Ofast} \\ \hline
\multicolumn{1}{l|}{Inst Boun} & \multicolumn{1}{l|}{\system} &  &  &  &  &  &  &  &  \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & \multirow{-2}{*}{-} & \multirow{-2}{*}{0.899} & \multirow{-2}{*}{0.868} & \multirow{-2}{*}{0.878} & \multirow{-2}{*}{0.889} & \multirow{-2}{*}{-} & \multirow{-2}{*}{-} & \multirow{-2}{*}{-} \\ \hline
\multicolumn{1}{l|}{Func Boun} & \multicolumn{1}{l|}{\system} & \textbf{0.974} & \textbf{0.985} & \textbf{0.936} & \textbf{0.981} & \textbf{0.959} & \textbf{0.889} & \textbf{0.615} & - \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & 0.663 & 0.424 & 0.448 & 0.362 & 0.418 & 0.554 & 0.688 & - \\ \hline
\multicolumn{1}{l|}{Func Sig Count} & \multicolumn{1}{l|}{\system} & \textbf{0.547} & - & \textbf{0.589} & - & \textbf{0.649} & \textbf{0.656} & \textbf{0.658} & \textbf{0.651} \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & { 0.501} & - & { 0.536} & - & { 0.582} & 0.578 & { 0.579} & 0.569 \\ \hline
\multicolumn{1}{l|}{Func Sig Type} & \multicolumn{1}{l|}{\system} & \textbf{0.829} & - & \textbf{0.729} & - & \textbf{0.757} & \textbf{0.745} & \textbf{0.758} & \textbf{0.758} \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & 0.529 & - & 0.532 & - & 0.548 & 0.537 & 0.543 & 0.539 \\ \hline
\multicolumn{1}{l|}{Func Name} & \multicolumn{1}{l|}{\system} & \textbf{0.826} & - & \textbf{0.835} & - & \textbf{0.839} & - & \textbf{0.837} & - \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & 0.645 & - & 0.663 & - & 0.667 & - & 0.675 & - \\ \hline
\multicolumn{1}{l|}{Comp Prov} & \multicolumn{1}{l|}{\system} & \textbf{0.92} & - & \textbf{0.559} & - & \textbf{0.238} & \textbf{0.488} & \textbf{0.287} & 0.258 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & 0.909 & - & 0.462 & - & 0.184 & 0.42 & 0.19 & \textbf{0.273} \\ \hline
 &  & \multicolumn{6}{c}{\textbf{Optimization Pair}} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
 &  & \textbf{O0,O3} & \textbf{O1,O3} & \textbf{O2,O3} & \textbf{O0,Os} & \textbf{O1,Os} & \textbf{O2,Os} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{l|}{Func Sim 32} & \multicolumn{1}{l|}{\system} & \textbf{0.796} & \textbf{0.943} & \textbf{0.973} & \textbf{0.84} & \textbf{0.944} & \textbf{0.941} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & 0.613 & 0.841 & 0.92 & 0.681 & 0.846 & 0.841 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{l|}{Func Sim 10000} & \multicolumn{1}{l|}{\system} & \textbf{0.218} & \textbf{0.619} & \textbf{0.792} & \textbf{0.256} & \textbf{0.592} & \textbf{0.614} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{XDA} & 0.085 & 0.305 & 0.596 & 0.095 & 0.283 & 0.328 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\end{tabular}%
}
\label{tab: RQ2_robustness_opt}
\end{table}

==> files/tables/RQ4_epochs.tex <==
\begin{table}[t]
\centering
\caption{The required number of fine-tuning epochs by XDA and \system to surpass the validation score threshold.}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{l|l|rrrrr}
\hline
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{l}{\textbf{Validation Score Threshold}} \\
 &  & \multicolumn{1}{l}{\textbf{0.9}} & \multicolumn{1}{l}{\textbf{0.7}} & \multicolumn{1}{l}{\textbf{0.5}} & \multicolumn{1}{l}{\textbf{0.3}} & \multicolumn{1}{l}{\textbf{0.1}} \\ \hline
Inst Boun & XDA & - & 1 & 1 & 1 & 1 \\
 & \system & - & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
Func Boun & XDA & - & - & - & 1 & 1 \\
 & \system & \textbf{15} & \textbf{4} & \textbf{2} & \textbf{1} & \textbf{1} \\ \hline
Comp Prov & XDA & - & - & - & 25 & 5 \\
 & \system & - & - & - & \textbf{8} & \textbf{2} \\ \hline
Mal CLS & XDA & - & 40 & 10 & 5 & 1 \\
 & \system & - & \textbf{10} & \textbf{5} & \textbf{3} & \textbf{1} \\ \hline
Func Sig Count & XDA & - & - & 37 & 10 & 3 \\
 & \system & - & \textbf{20} & \textbf{9} & \textbf{3} & \textbf{1} \\ \hline
Func Sig Type & XDA & - & - & 39 & 18 & 1 \\
 & \system & - & - & \textbf{19} & \textbf{7} & \textbf{1} \\ \hline
Func Name & XDA & - & - & 66 & 44 & 28 \\
 & \system & - & \textbf{61} & \textbf{37} & \textbf{23} & \textbf{10} \\ \hline
Func Sim 32 & XDA & - & 1 & 1 & 1 & 1 \\
 & \system & \textbf{25} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\ \hline
Func Sim 10000 & XDA & - & - & - & - & 1 \\
 & \system & - & - & 20 & \textbf{1} & \textbf{1} \\ \hline
\end{tabular}%
}
\label{tab: RQ4_training_epochs}
\end{table}

==> files/tables/abbreviation.tex <==
\begin{table}[h]
\centering
\caption{Task Abbreviation references.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l}
\hline
Abbreviation & Full Task Name \\ \hline
Inst Boun & Instruction boundary recovery \\
Func Boun & Function boundary recovery \\
Func Sig Count & Function signature prediction (\# of arguments) \\
Func Sig Type & Function signature prediction (return type) \\
Func Name & Function name prediction \\
Comp Prov & Compiler provenance \\
Func Sim 32/10000 & Function Similarity Detection (pool size 32/10000) \\ \hline
\end{tabular}%
}
\label{tab: task abbreviation}
\end{table}

==> files/tables/prevmodels.tex <==
\begin{table*}[th!]
\centering
\caption{Properties of existing Binary Code Embedding (BCE) approaches and their comparison with \system.}
\label{tab:prevstudy}
\begin{threeparttable}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccclcccccccccc}
\hline
 &  & \multicolumn{9}{c}{\textbf{Transformer-based}} &  & \multicolumn{9}{c}{\textbf{RNN/CNN/GNN-based}} & \multicolumn{1}{l}{} \\ \cline{3-11} \cline{13-21}
 &  & \rotatebox[origin=l]{90}{XDA} & \rotatebox[origin=l]{90}{Binprov} & \rotatebox[origin=l]{90}{Palmtree} & \rotatebox[origin=l]{90}{jTrans} & \rotatebox[origin=l]{90}{kTrans} & \rotatebox[origin=l]{90}{Trex} & \rotatebox[origin=l]{90}{Symlm} & \rotatebox[origin=l]{90}{CodeArt} & \rotatebox[origin=l]{90}{BinBert} &  & \rotatebox[origin=l]{90}{Malconv2} & \rotatebox[origin=l]{90}{DeepDi} & \rotatebox[origin=l]{90}{Bi-RNN} & \rotatebox[origin=l]{90}{EKLAVYA} & \rotatebox[origin=l]{90}{XFL} & \rotatebox[origin=l]{90}{Structure2Vec } & \rotatebox[origin=l]{90}{SAFE} & \rotatebox[origin=l]{90}{Gemini} & \rotatebox[origin=l]{90}{Nimbus} & \rotatebox[origin=l]{90}{\system} \\
 &  & \cite{pei2020xda} & \cite{he2022binprov} & \cite{li2021palmtree} & \cite{wang2022jtrans} & \cite{zhu2023ktrans} & \cite{pei2020trex} & \cite{jin2022symlm} & \cite{su2024codeart} & \cite{artuso2024binbert} &  & \cite{raff2021classifying} & \cite{yu_deepdi_2022} & \cite{shin2015recognizing} & \cite{chua2017neural} & \cite{patrick2023xfl} & \cite{massarelli2019investigating} & \cite{massarelli2019safe} & \cite{xu2017neural} & \cite{qian2022nimbus} & $\bigstar$ \\ \hline
 & Raw Byte & \newmoon & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ &  & \newmoon & \RIGHTcircle & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon \\
 & Assembly & $\cdot$ & $\cdot$ & \newmoon & \newmoon & \newmoon & \newmoon & \newmoon & \newmoon & \newmoon &  & $\cdot$ & \RIGHTcircle & $\cdot$ & \newmoon & \newmoon & \newmoon & \newmoon & \newmoon & \newmoon & $\cdot$ \\
 & CFG & $\cdot$ & $\cdot$ & \newmoon & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ \\
 & DFG & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ \\
 & Register Info & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ \\
 & Operand Info & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ \\
 & Caller/Callee Info & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ \\
\multirow{-8}{*}{\textbf{Input Modality}} & Dynamic Behavior & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & \newmoon & $\cdot$ & \newmoon &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ \\ \hline
 & Disassembly & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ &  & $\cdot$ & \newmoon & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon \\
 & Compiler Provenance & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon \\
 & Malware Classification & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ &  & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon \\
 & Function Signature & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & \newmoon \\
 & Function Name & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & \newmoon &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon \\
\multirow{-6}{*}{\textbf{Binary Task}} & Function Similarity & $\cdot$ & $\cdot$ & \newmoon & \newmoon & \newmoon & \newmoon & $\cdot$ & \newmoon & $\cdot$ &  & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & \newmoon & \newmoon & \newmoon & $\cdot$ & \newmoon \\ \hline
\multicolumn{2}{l}{Equipped with Binary Code Knowledge} & $\cdot$ & $\cdot$ & \RIGHTcircle & \RIGHTcircle & \RIGHTcircle & \RIGHTcircle & \RIGHTcircle & \RIGHTcircle & \RIGHTcircle &  & $\cdot$ & \RIGHTcircle & $\cdot$ & $\cdot$ & \RIGHTcircle & \RIGHTcircle & $\cdot$ & \RIGHTcircle & $\cdot$ & \newmoon \\
\multicolumn{2}{l}{No Feature Engineering} & \newmoon & \newmoon & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ & $\cdot$ &  & \newmoon & $\cdot$ & \newmoon & \newmoon & $\cdot$ & $\cdot$ & \newmoon & $\cdot$ & \newmoon & \newmoon \\ \hline
\end{tabular}%
}
    \begin{tablenotes}
    \item [\newmoon] This mark denotes the feature is fully implemented in the model.
    \item [\RIGHTcircle] This mark denotes that the model has a partial implementation of this feature.
    \end{tablenotes}
\end{threeparttable}
\end{table*}

==> files/tables/try.tex <==

\begin{table*}
\begin{minipage}{\columnwidth}
    \centering
    \begin{tabular}{|c|c|}
      \hline 1 & 2 \\ \hline 3 & 4 \\ \hline
    \end{tabular}
    \caption{table 1}
\end{minipage}\hfill 
\begin{minipage}{\columnwidth}
    \centering
    \begin{tabular}{|c|c|}
      \hline 1 & 2 \\ \hline 3 & 4 \\ \hline
    \end{tabular}
    \caption{table 2}
  \end{minipage}
\end{table*}
